Relativistic Entropy Inequality

In this paper we apply the entropy principle to the relativistic version of the differential equations describing a standard fluid flow, that is, the equations for mass, momentum, and a system for the energy matrix. These are the second order equations which have been introduced in [3]. Since the principle also says that the entropy equation is a scalar equation, this implies, as we show, that one has to take a trace in the energy part of the system. Thus one arrives at the relativistic mass-momentum-energy system for the fluid. In the procedure we use the well-known Liu-M\"uller sum [10] in order to deduce the Gibbs relation and the residual entropy inequality.

==> Alt-entropy-arXiv.tex <==
%&latex
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Relativistic entropy inequality
%%  Article by Prof. H.W. Alt
%%  Copyright 2017-2017 by H. W. Alt
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Languages
\newcommand{\DE}[1]{}
\newcommand{\EN}[1]{#1}
%%
%% PDF-version
\newcommand{\PDF}[2]{#2} % in script.sty
%%
%% Nocolor
\newif\ifnocolor
\nocolortrue
%% Nonewpage
%% Final version
\newif\iffinal
\finaltrue
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LaTeX-Dokument
\input{./TITELEI/dynamo-AMSA.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> LATEX/greek-hyp.tex <==
%% -*-Latex-*-
%%

The pronounciation of mathematical formulas requires
the knowledge of the Greek alphabet.\\
The following table serves as a check, whether your browser
is able to represent these letters.\\
\begin{comment}
Das Aussprechen mathematischer Formeln erfordert die Kenntnis des
Griechischen Alphabets:
\end{comment}

\xml{table align="center" border="6" cellpadding="8" rules="all" bgcolor="#8888ff"}
\xml{thead}\xml{tr}\xml{td colspan="3" align="center"}Greek Alphabet\xml{/td}\xml{/tr}\xml{/thead}
\xml{tbody}
\xml{tr}
\xml{td}alpha\xml{/td}\xml{td}$\alpha$\xml{/td}\xml{td}$\Alpha$, $A$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}beta\xml{/td}\xml{td}$\beta$\xml{/td}\xml{td}$\Beta$, $B$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}gamma\xml{/td}\xml{td}$\gamma$\xml{/td}\xml{td}$\Gamma$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}delta\xml{/td}\xml{td}$\delta$\xml{/td}\xml{td}$\Delta$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}epsilon\xml{/td}\xml{td}$\stdepsilon$, $\altepsilon$\xml{/td}\xml{td}$\Eps$, $E$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}zeta\xml{/td}\xml{td}$\zeta$\xml{/td}\xml{td}$\Zeta$, $Z$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}eta\xml{/td}\xml{td}$\eta$\xml{/td}\xml{td}$\Eta$, $H$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}theta\xml{/td}\xml{td}$\theta$, $\alttheta$\xml{/td}\xml{td}$\Theta$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}iota\xml{/td}\xml{td}$\iota$\xml{/td}\xml{td}$\Iota$, $I$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}kappa\xml{/td}\xml{td}$\stdkappa$, $\altkappa$\xml{/td}\xml{td}$\Kappa$, $K$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}lambda\xml{/td}\xml{td}$\lambda$\xml{/td}\xml{td}$\Lambda$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}mu\xml{/td}\xml{td}$\mu$\xml{/td}\xml{td}$\Mu$, $M$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}nu\xml{/td}\xml{td}$\nu$\xml{/td}\xml{td}$\Nu$, $N$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}xi\xml{/td}\xml{td}$\xi$\xml{/td}\xml{td}$\Xi$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}omicron\xml{/td}\xml{td}$\omicron$, $o$\xml{/td}\xml{td}$\Omicron$, $O$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}pi\xml{/td}\xml{td}$\pi$\xml{/td}\xml{td}$\Pi$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}rho\xml{/td}\xml{td}$\stdrho$, $\altrho$\xml{/td}\xml{td}$\Rho$, $P$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}sigma\xml{/td}\xml{td}$\stdsigma$, $\altsigma$\xml{/td}\xml{td}$\Sigma$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}tau\xml{/td}\xml{td}$\tau$\xml{/td}\xml{td}$\Tau$, $T$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}ypsilon\xml{/td}\xml{td}$\upsilon$\xml{/td}\xml{td}$\Upsilon$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}phi\xml{/td}\xml{td}$\stdphi$, $\altphi$\xml{/td}\xml{td}$\Phi$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}chi\xml{/td}\xml{td}$\chi$\xml{/td}\xml{td}$\Chi$, $X$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}psi\xml{/td}\xml{td}$\psi$\xml{/td}\xml{td}$\Psi$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}omega\xml{/td}\xml{td}$\omega$\xml{/td}\xml{td}$\Omega$\xml{/td}
\xml{/tr}
\xml{/tbody}
\xml{/table}

%-------------------------------------------------------


==> LATEX/mathsymbols-hyp.tex <==
%% -*-Latex-*-
%%

The following tables serve as a check, whether your browser
is able to represent mathematical symbols.
First a list of some very basic symbols.

\xml{table align="center" border="6" cellpadding="8" rules="all" bgcolor="#8888ff"}
\xml{thead}\xml{tr}\xml{td colspan="2" align="center"}Mathematical Symbols\xml{/td}\xml{/tr}\xml{/thead}
\xml{tbody}
\xml{tr}
\xml{td}union\xml{/td}\xml{td}$\cup$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}intersection\xml{/td}\xml{td}$\cap$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}element of\xml{/td}\xml{td}$\in$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}subset of\xml{/td}\xml{td}$\subset$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}empty set\xml{/td}\xml{td}$\emptyset$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}infinity\xml{/td}\xml{td}$\infty$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}greater or equal\xml{/td}\xml{td}$\geq$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}sum\xml{/td}\xml{td}$\sum$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}product\xml{/td}\xml{td}$\prod$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}integral\xml{/td}\xml{td}$\int$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}perpendicular\xml{/td}\xml{td}$\perp$\xml{/td}
\xml{/tr}
\xml{/tbody}
\xml{/table}

Here a more detailed list of very often used mathematical symbols.

\xml{table align="center" border="6" cellpadding="8" rules="all" bgcolor="#8888ff"}
\xml{thead}
\xml{tr}
\xml{td colspan="4" align="center"}Mathematical Symbols\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}LaTeX\xml{/td}\xml{td}Unicode\xml{/td}
\xml{td}Name\xml{/td}\xml{td}Your Browser\xml{/td}
\xml{/tr}
\xml{/thead}
\xml{tbody}
\xml{tr}
\xml{td}\backslash cup\xml{/td}\xml{td}222A\xml{/td}
\xml{td}union\xml{/td}\xml{td}$\cup$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash cap\xml{/td}\xml{td}2229\xml{/td}
\xml{td}intersection\xml{/td}\xml{td}$\cap$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash in\xml{/td}\xml{td}2208\xml{/td}
\xml{td}element of\xml{/td}\xml{td}$\in$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash notin\xml{/td}\xml{td}2209\xml{/td}
\xml{td}not element of\xml{/td}\xml{td}$\notin$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash subset\xml{/td}\xml{td}2282\xml{/td}
\xml{td}subset of\xml{/td}\xml{td}$\subset$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash setminus\xml{/td}\xml{td}2216\xml{/td}
\xml{td}set difference\xml{/td}\xml{td}$\setminus$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash emptyset\xml{/td}\xml{td}2205\xml{/td}
\xml{td}empty set\xml{/td}\xml{td}$\emptyset$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash infty\xml{/td}\xml{td}221E\xml{/td}
\xml{td}infinity\xml{/td}\xml{td}$\infty$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash geq, \backslash ge\xml{/td}\xml{td}2267 (2265)\xml{/td}
\xml{td}greater or equal\xml{/td}\xml{td}$\geq$ (\unicode{2265})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash leq, \backslash le\xml{/td}\xml{td}2266 (2264)\xml{/td}
\xml{td}less or equal\xml{/td}\xml{td}$\leq$ (\unicode{2264})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash neq\xml{/td}\xml{td}2260\xml{/td}
\xml{td}not equal\xml{/td}\xml{td}$\neq$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash sum\xml{/td}\xml{td}2211\xml{/td}
\xml{td}sum\xml{/td}\xml{td}$\sum$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash prod\xml{/td}\xml{td}220F\xml{/td}
\xml{td}product\xml{/td}\xml{td}$\prod$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash int\xml{/td}\xml{td}222B\xml{/td}
\xml{td}integral\xml{/td}\xml{td}$\int$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash perp\xml{/td}\xml{td}22A5\xml{/td}
\xml{td}perpendicular\xml{/td}\xml{td}$\perp$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash forall\xml{/td}\xml{td}2200\xml{/td}
\xml{td}for all\xml{/td}\xml{td}$\forall$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash exists\xml{/td}\xml{td}2203\xml{/td}
\xml{td}there exists\xml{/td}\xml{td}$\exists$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash partial\xml{/td}\xml{td}2202\xml{/td}
\xml{td}partial derivative\xml{/td}\xml{td}$\partial$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash nabla\xml{/td}\xml{td}2207\xml{/td}
\xml{td}nabla operator\xml{/td}\xml{td}$\nabla$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash wedge\xml{/td}\xml{td}2227\xml{/td}
\xml{td}wedge product\xml{/td}\xml{td}$\wedge$\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash circ\xml{/td}\xml{td}2218\xml{/td}
\xml{td}composition\xml{/td}\xml{td}$\circ$\xml{/td}
\xml{/tr}
\xml{tr}
%\xml{td}\backslash to (\backslash rightarrow)\xml{/td}\xml{td}2192\xml{/td}
\xml{td}\backslash to\xml{/td}\xml{td}2192\xml{/td}
\xml{td}converges to\xml{/td}\xml{td}\unicode{2192}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash mapsto\xml{/td}\xml{td}21A6 (27FC)\xml{/td}
\xml{td}maps to\xml{/td}\xml{td}\unicode{21a6} (\unicode{27fc})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash nearrow\xml{/td}\xml{td}2197\xml{/td}
\xml{td}north east arrow\xml{/td}\xml{td}\unicode{2197}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash searrow\xml{/td}\xml{td}2198\xml{/td}
\xml{td}south east arrow\xml{/td}\xml{td}\unicode{2198}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash pm\xml{/td}\xml{td}00B1\xml{/td}
\xml{td}plus minus\xml{/td}\xml{td}\unicode{b1}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash mp\xml{/td}\xml{td}2213\xml{/td}
\xml{td}minus plus\xml{/td}\xml{td}\unicode{2213}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash vdots\xml{/td}\xml{td}22EE\xml{/td}
\xml{td}vertical dots\xml{/td}\xml{td}\unicode{22ee}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash ddots\xml{/td}\xml{td}22F1\xml{/td}
\xml{td}diagonal dots\xml{/td}\xml{td}\unicode{22f1}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash langle\xml{/td}\xml{td}2329 (003C)\xml{/td}
\xml{td}left angle\xml{/td}\xml{td}\unicode{2329} (\unicode{3c})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash rangle\xml{/td}\xml{td}232A (003A)\xml{/td}
\xml{td}right angle\xml{/td}\xml{td}\unicode{232a} (\unicode{3e})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash |\xml{/td}\xml{td}2016 (2225)\xml{/td}
\xml{td}double vertical line\xml{/td}\xml{td}\unicode{2016} (\unicode{2225})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash bullet\xml{/td}\xml{td}2219 (2022)\xml{/td}
\xml{td}bullet operator\xml{/td}\xml{td}\unicode{2219} (\unicode{2022})\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash oplus\xml{/td}\xml{td}2295\xml{/td}
\xml{td}circled plus\xml{/td}\xml{td}\unicode{2295}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash otimes\xml{/td}\xml{td}2297\xml{/td}
\xml{td}circled times\xml{/td}\xml{td}\unicode{2297}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash sim\xml{/td}\xml{td}223C\xml{/td}
\xml{td}similar to\xml{/td}\xml{td}\unicode{223c}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash approx\xml{/td}\xml{td}2248\xml{/td}
\xml{td}asymptotic to\xml{/td}\xml{td}\unicode{2248}\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash tilde\{x\}\xml{/td}\xml{td}0078+0303\xml{/td}
\xml{td}combining tilde\xml{/td}\xml{td}\unicode{78}\unicode{303}
%, \begin{rawxml}&#x78&#x303;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash tilde\{M\}\xml{/td}\xml{td}004D+0303\xml{/td}
\xml{td}combining tilde\xml{/td}\xml{td}\unicode{4d}\unicode{303}
%, \begin{rawxml}&#x4d&#x303;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash bar\{x\}\xml{/td}\xml{td}0078+0305\xml{/td}
\xml{td}combining overline\xml{/td}\xml{td}\unicode{78}\unicode{305}
%, \begin{rawxml}&#x78&#x305;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash bar\{M\}\xml{/td}\xml{td}004D+0305\xml{/td}
\xml{td}combining overline\xml{/td}\xml{td}\unicode{4d}\unicode{305}
%, \begin{rawxml}&#x4d&#x305;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash hat\{x\}\xml{/td}\xml{td}0078+0302\xml{/td}
\xml{td}combining circumflex\xml{/td}\xml{td}\unicode{78}\unicode{302}
%, \begin{rawxml}&#x78&#x302;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash hat\{M\}\xml{/td}\xml{td}004D+0302\xml{/td}
\xml{td}combining circumflex\xml{/td}\xml{td}\unicode{4d}\unicode{302}
%, \begin{rawxml}&#x4d&#x302;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
\xml{tr}
\xml{td}\backslash not\{O\}\xml{/td}\xml{td}004F+0338\xml{/td}
\xml{td}combining slash\xml{/td}\xml{td}\unicode{4f}\unicode{338}
%, \begin{rawxml}&#x4d&#x302;\end{rawxml}\xml{/td}
\xml{/td}
\xml{/tr}
%\xml{tr}
%\xml{td}real numbers\xml{/td}\xml{td}$\RR$\xml{/td}
%\xml{/tr}
% add real numbers
% add prime
% add dot
% add \frac
\xml{/tbody}
\xml{/table}

In the last combining symbols the tilde, bar, and hat
should be placed on top of the characters 'x' and 'M'.

%-------------------------------------------------------




==> LATEX/translate.tex <==
%% -*-latex-*-
%%

%% Some useful language switches (used only in formulas)
\DE{\newcommand{\fast}{fast }}
\EN{\newcommand{\fast}{almost }}
\DE{\newcommand{\ueberall}{\"uberall }}
\EN{\newcommand{\ueberall}{everywhere }}
\DE{\newcommand{\wenn}{f\"ur }}
\EN{\newcommand{\wenn}{as }}
\DE{\newcommand{\fuer}{f\"ur }}
\EN{\newcommand{\fuer}{for }}
\DE{\newcommand{\alle}{alle }}
\EN{\newcommand{\alle}{all }}
\DE{\newcommand{\und}{und }}
\EN{\newcommand{\und}{and }}
\DE{\newcommand{\wobei}{wobei }}
\EN{\newcommand{\wobei}{where }}
\DE{\newcommand{\jedoch}{jedoch }}
\EN{\newcommand{\jedoch}{but }}
\DE{\newcommand{\lokal}{lokal }}
\EN{\newcommand{\lokal}{locally }}
\DE{\newcommand{\siehe}{siehe }}
\EN{\newcommand{\siehe}{see }}
\DE{\newcommand{\von}{von }}
\EN{\newcommand{\von}{of }}
\DE{\newcommand{\auf}{auf }}
\EN{\newcommand{\auf}{on }}
%\show\mit % already defined !!!
%\DE{\newcommand{\mit}{mit }}
%\EN{\newcommand{\mit}{whith }}


